Hyperbolic tilings and formal language theory

In this paper, we try to give the appropriate class of languages to which belong various objects associated with tessellations in the hyperbolic plane.

==> eptcsdata.tex <==
\providecommand{\firstpage}{126}
\providecommand{\publicationstatus}{T. Neary and M. Cook (Eds.):\\
Machines, Computations and Universality (MCU 2013)\\
EPTCS 128, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.128.18}{10.4204/EPTCS.128.18}}

